Scaling Properties of Continuous Diffusion Spoken Language Models

Speech-only spoken language models (SLMs) lag behind text and text-speech models in performance, with recent discrete autoregressive (AR) SLMs indicating significant computational and data demands to match text models. Since discretizing continuous speech for AR creates bottlenecks, we explore whether continuous diffusion (CD) SLM is more viable. To quantify the SLMs linguistic quality, we introduce the phoneme Jensen-Shannon divergence (pJSD) metric. Our analysis reveals CD SLMs, mirroring AR behavior, exhibit scaling laws for validation loss and pJSD, and show optimal token-to-parameter ratios decreasing as compute scales. However, for the latter, loss becomes insensitive to choice of data and model sizes, showing potential for fast inference. Scaling CD SLMs to 16B parameters with tens of millions of hours of conversational data enables generation of emotive, prosodic, multi-speaker, multilingual speech, though achieving long-form coherence remains a significant challenge.

==> body/03_04_ablations.tex <==
\section{Continuous Diffusion SLMs Ablations}
\label{sec:ablations}
%
\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{plotting/ablation_cross_comparison.pdf}
  \caption{Ablation Summary.}
  \label{fig:ablation_summary}
\end{figure}
%
To evaluate the sensitivity of our model to key design choices, we conduct systematic ablations across temporal resolution, diffusion discretization, and noise scheduling. We assess these configurations using the 
%perceptual, aesthetic, and phonetic 
metrics detailed in~\Cref{sec:perception-metrics}. For these ablations we also incorporate the Frechet Audio Distance (FAD) metric. We observe that FAD exhibits considerable noise and frequently diverges from perceptual consensus within our continuous framework. Consequently, we advise interpreting its fluctuations with caution and prioritize reference-free estimators and aesthetic scores in our analysis. All base models are trained with 8 layers and $d_{\text{emb}}=1024$, and evaluated at weak and strong classifier-free guidance scales. We use CompleteP \cite{dey2025dont} to transfer the base hyperparameters to other model sizes. ~\Cref{fig:ablation_summary} summaarizes the result of all ablations.

\subsection{Fixed model, growing data}
%
\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{plotting/ablation_duration.pdf}
  \caption{Effect of training duration on audio quality. Subjective metrics improve monotonically with increased audio data.}
  \label{fig:ablation_duration}
\end{figure}
%
Generation quality scales predictably with training compute. As shown in Figure~\ref{fig:ablation_duration}, subjective quality metrics improve monotonically as training progresses from 0.25M to 1.5M hours of audio. In contrast, FAD saturates prematurely and fluctuates, further reinforcing our caution regarding its reliability as a consistent quality indicator.

\subsection{Patching log mel-filterbanks} 
%
\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{plotting/ablation_mel_folds.pdf}
  \caption{Effect of temporal patch size on audio quality. Smaller patches preserve fine-grained temporal structure, yielding consistently better perceptual quality.}
  \label{fig:ablation_patch_size}
\end{figure}
%
We investigate folding the log mel-filterbank temporal dimension into channels to reduce sequence length. Figure~\ref{fig:ablation_patch_size} demonstrates that a patch size of 1 preserves fine-grained temporal structure, yielding the highest perceptual and aesthetic scores. Larger patch sizes exhibit progressive quality degradation, highlighting the necessity of high temporal resolution for high-fidelity speech generation.
%
\subsection{Diffusion Timestep Discretization}
For diffusion timestep discretization ($T$), preliminary observations indicate a modest advantage at $T=500$ within our experimental conditions (Figure~\ref{fig:ablation_timesteps}). However, performance variations around this value are minor and not strictly monotonic, suggesting that $T=500$ represents a practical compromise rather than a definitive optimum. Further experimentation would be necessary to robustly characterize the relationship between discretization granularity and generation quality.
%
\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{plotting/ablation_num_timesteps.pdf}
  \caption{Effect of diffusion timesteps $T$ on audio quality. 
  % An optimum emerges at $T=500$, with both coarser and finer discretizations yielding degraded performance.
  }
  \label{fig:ablation_timesteps}
\end{figure}

\subsection{Noise Scheduling and Guidance}
\label{sec:ablation_noise_schedule}
%
\widetemplatefigurebegin
  \centering
  \includegraphics[width=\linewidth]{plotting/ablation_noise_schedule_cfg2.2.pdf}
  \caption{Noise schedule ablation at weak guidance. Each cell is a separately trained model and shows the metric value for a schedule type and terminal SNR setting. Black borders indicate optimal configurations. In this regime the exponential schedule training dominates.}
  \label{fig:ablation_noise_cfg22}
\widetemplatefigureend
%
\widetemplatefigurebegin
  \centering
  \includegraphics[width=\linewidth]{plotting/ablation_noise_schedule_cfg4.0.pdf}
  \caption{Under strong guidance, linear schedules (especially with zero terminal SNR) dominate most perceptual and aesthetic metrics, while exponential schedules no longer lead.}
  \label{fig:ablation_noise_cfg40}
\widetemplatefigureend
%
The noise schedule, which dictates the signal-to-noise ratio progression, is best interpreted jointly with the intended inference guidance regime (Figures~\ref{fig:ablation_noise_cfg22} and~\ref{fig:ablation_noise_cfg40}). Across configurations, we observe that the cosine schedule consistently trails linear and exponential alternatives.
%
Beyond this, the optimal schedule diverges based on the sampling regime. Under weak guidance (CFG 2), exponential schedules tend to achieve better aesthetic scores. However, under stronger guidance (CFG 4), a linear schedule combined with zero terminal SNR (enforcing complete signal destruction at $t=T$) emerges as the most robust choice across phonetic and perceptual metrics. This shift suggests that stronger guidance may amplify sensitivity to modeling errors at high noise levels, thereby favoring schedules that explicitly support early, high-noise denoising.


==> body/03_05_ablations_v2.tex <==
\section{Continuous Diffusion SLMs Ablations} 
\label{sec:ablation_summary} 
% %
%
\begin{figure}[htbp] 
  \centering 
  \includegraphics[width=\linewidth]{plotting/ablation_cross_comparison.pdf} 
  \caption{Cross-ablation metric distributions. Diffusion dynamics (noise schedules) dominate perception quality, while data scale (duration) drives languageness.} 
  \label{fig:ablation_cross} 
\end{figure}
%
To understand the sensitivity of our continuous diffusion SLM to different design choices, we conduct a systematic ablation study across three semantic axes: data scale, diffusion dynamics, and architectural compression. All base models feature 8 layers and $d_{\text{emb}}=1024$, with hyperparameters tuned using a sweep over learning rate, weight decay, and Adam parameters ($\beta_1, \beta_2$, $\epsilon$) and are evaluated under both weak and strong \gls{cfg}. We use completeP \cite{dey2025dont} to transfer the base hyperparameters to other model sizes. Figure~\ref{fig:ablation_cross} synthesizes the metric distributions across these studies.

\textbf{Data Scale (Training Duration):} 
We varied cumulative training audio from 0.25M to 1.5M hours. 
\textit{Takeaway:} Scale is the primary driver of ``languageness'' and semantic capabilities (content enjoyment and understanding), aligning with our core scaling laws.

\textbf{Diffusion Dynamics (Schedules \& Timesteps):} 
We evaluated linear, cosine, and exponential noise schedules (with and without zero terminal SNR \cite{DBLP:conf/wacv/LinLLY24}), alongside training timestep discretizations $T \in \{100, 500, 1000, 2000, 4000\}$. 
\textit{Takeaway:} Noise schedules strictly dictate perceptual quality and signal fidelity. The cosine schedule consistently underperforms. Conversely, pairing a linear schedule with zero terminal SNR excels by explicitly enforcing signal destruction, improving robustness in high-noise regimes.

\textbf{Architectural Compression (Temporal Patch Size $k$):} 
We folded the temporal dimension by $k \in \{1, \dots, 6\}$ to reduce sequence length and compute. 
\textit{Takeaway:} Increasing $k$ uniformly degrades all metrics. This underscores that fine grained temporal resolution is critical for high-fidelity audio and natural prosody, outweighing the computational savings of larger patches.


==> body/97_temporary_devlog_fitting_scaling_laws.tex <==
\clearpage
\subsection{[Temporary][Devlog] Fitting Scaling Laws}
\label{sec:temporary-devlog-fitting-scaling-laws}


\subsubsection{Scaling Law for Validation Loss}
\label{sec:temporary-devlog-fitting-scaling-laws:scaling-law-for-validation-loss}
\noindent Following the literature, we attempt to fit a scaling law for the validation loss $L$ of the models using the functional form:
\begin{equation}
    \label{eq:temporary-devlog-fitting-scaling-laws:scaling-law-for-validation-loss:base-scaling-law-expression}
    L 
    =
    % \underbrace{E}_{\textrm{Irreducible term}}
    E 
    + 
    \left(
        \frac{A}{N^\alpha}
        +
        \frac{B}{D^\beta}
    \right)^\gamma
\end{equation}
\noindent We observed that parameterizing the overall power $\gamma$ is necessary to get a good scaling law fit with low enough MRE and thus, we chose the functional form of $\Cref{eq:temporary-devlog-fitting-scaling-laws:scaling-law-for-validation-loss:base-scaling-law-expression}$ rather than the vanilla form $L = E + \frac{A}{N^\alpha} + \frac{B}{D^\beta}$. 
\begin{figure}[ht]
    \centering
    % \includegraphics[width=0.49\textwidth]
    \includegraphics[width=\linewidth]{plotting/000004_scaling_law_fits/eval_loss_min_snr_avg/isoflop_curves_vs_D.png}
    \caption{
        Scaling law fit for validation loss.
    }
    \label{fig:000004_scaling_law_fits:eval_loss_min_snr_avg:isoflop_curves_vs_D.png}
\end{figure}

\noindent The coefficients of the best scaling law fit we find with our optimization setup are shown in~\Cref{tab:000004_scaling_law_fits:eval_loss_min_snr_avg:scaling_law_coefficients}.
\begin{table}[!ht]
\centering
\caption{Fitted coefficients for the scaling law $L(N,D) = E + (A / N^{\alpha} + B / D^{\beta})^{\gamma}$ on \texttt{eval\_loss\_min\_snr\_avg}.}
\label{tab:000004_scaling_law_fits:eval_loss_min_snr_avg:scaling_law_coefficients}
\begin{tabular}{@{}cccccc@{}}
\toprule
$E$ & $A$ & $B$ & $\alpha$ & $\beta$ & $\gamma$ \\
\midrule
$0.0055$ & $0.0612$ & $16.2179$ & $0.4226$ & $0.5531$ & $0.6745$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!ht]
\footnotesize
\centering
\caption{Compute-optimal allocation for \texttt{eval\_loss\_min\_snr\_avg}. For each compute budget $C$, we report the optimal model size $N^\ast$, optimal number of tokens $D^*$, and optimal tokens-per-parameter ratio $r^* = D^*/N^*$.}
\label{tab:000004_scaling_law_fits:eval_loss_min_snr_avg:compute_optimal_training_details}
\begin{tabular}{@{}cccc@{}}
\toprule
Compute $C$ & $N^*$ & $D^*$ & $r^*$ \\
\midrule
$1\mathrm{e}{18}$ & $1.44\mathrm{e}{7}$ & $1.16\mathrm{e}{10}$ & 801 \\
\cmidrule{1-4}
$3\mathrm{e}{18}$ & $2.69\mathrm{e}{7}$ & $1.86\mathrm{e}{10}$ & 692 \\
\cmidrule{1-4}
$6\mathrm{e}{18}$ & $3.98\mathrm{e}{7}$ & $2.51\mathrm{e}{10}$ & 631 \\
\cmidrule{1-4}
$1\mathrm{e}{19}$ & $5.32\mathrm{e}{7}$ & $3.13\mathrm{e}{10}$ & 589 \\
\cmidrule{1-4}
$3\mathrm{e}{19}$ & $9.92\mathrm{e}{7}$ & $5.04\mathrm{e}{10}$ & 509 \\
\cmidrule{1-4}
$6\mathrm{e}{19}$ & $1.47\mathrm{e}{8}$ & $6.81\mathrm{e}{10}$ & 464 \\
\cmidrule{1-4}
$1\mathrm{e}{20}$ & $1.96\mathrm{e}{8}$ & $8.49\mathrm{e}{10}$ & 433 \\
\cmidrule{1-4}
$3\mathrm{e}{20}$ & $3.66\mathrm{e}{8}$ & $1.37\mathrm{e}{11}$ & 374 \\
\cmidrule{1-4}
$6\mathrm{e}{20}$ & $5.42\mathrm{e}{8}$ & $1.85\mathrm{e}{11}$ & 341 \\
\cmidrule{1-4}
$1\mathrm{e}{21}$ & $7.24\mathrm{e}{8}$ & $2.30\mathrm{e}{11}$ & 319 \\
\bottomrule
\end{tabular}
\end{table}


\begin{figure}[ht]
    \centering
    % \includegraphics[width=0.49\textwidth]
    \includegraphics[width=\linewidth]{plotting/000004_scaling_law_fits/eval_loss_min_snr_avg/r_star_vs_C.png}
    \caption{
        Scaling law fit for validation loss.
    }
    \label{fig:000004_scaling_law_fits:eval_loss_min_snr_avg:r_star_vs_C}
\end{figure}


\begin{table*}[t]
\centering
\footnotesize
\caption{
    Analysis of flatness of the isoFLOPs near their optimality point. 
    For a given compute budget $C$, we show the range of model sizes $[N_1, N_2]$ and dataset sizes $[D_1, D2]$ while keeping the compute budget fixed to $C$ such that the corresponding loss prediction $L$ for these models lies in range $[L^\ast , L^\ast + \epsilon]$. 
    Here, $L^\ast$ would represent the optimal loss achievable with the given compute. 
    In addition, we plot the curvature of the isoFLOPs at their optimality points.
    These results indicate that as compute budget increases, the curvature of the isoFLOPs generally increases.
}
\label{tab:000004_scaling_law_fits:eval_loss_min_snr_avg:scaling_law_fits_curvature}
\begin{tabular}{@{}ccccccccc@{}}
\toprule
 & & \multicolumn{3}{c}{Model size $N$} & \multicolumn{3}{c}{Dataset size $D$} & \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
$C$ & $L^\ast$ & $N_1$ & $N_2$ & $\Delta N$ & $D_1$ & $D_2$ & $\Delta D$ & $\kappa$ \\
\midrule
$1\mathrm{e}{18}$ & $0.007486$ & $1.06\mathrm{e}{6}$ & $1.54\mathrm{e}{8}$ & $1.53\mathrm{e}{8}$ & $1.57\mathrm{e}{11}$ & $1.08\mathrm{e}{9}$ & $1.56\mathrm{e}{11}$ & $1.54\mathrm{e}{-18}$ \\
\cmidrule{1-9}
$3\mathrm{e}{18}$ & $0.007156$ & $1.54\mathrm{e}{6}$ & $3.52\mathrm{e}{8}$ & $3.50\mathrm{e}{8}$ & $3.24\mathrm{e}{11}$ & $1.42\mathrm{e}{9}$ & $3.23\mathrm{e}{11}$ & $3.70\mathrm{e}{-19}$ \\
\cmidrule{1-9}
$6\mathrm{e}{18}$ & $0.006976$ & $1.93\mathrm{e}{6}$ & $5.97\mathrm{e}{8}$ & $5.95\mathrm{e}{8}$ & $5.17\mathrm{e}{11}$ & $1.67\mathrm{e}{9}$ & $5.15\mathrm{e}{11}$ & $1.51\mathrm{e}{-19}$ \\
\cmidrule{1-9}
$1\mathrm{e}{19}$ & $0.006856$ & $2.27\mathrm{e}{6}$ & $8.86\mathrm{e}{8}$ & $8.84\mathrm{e}{8}$ & $7.34\mathrm{e}{11}$ & $1.88\mathrm{e}{9}$ & $7.32\mathrm{e}{11}$ & $7.79\mathrm{e}{-20}$ \\
\cmidrule{1-9}
$3\mathrm{e}{19}$ & $0.006628$ & $3.16\mathrm{e}{6}$ & $2.10\mathrm{e}{9}$ & $2.09\mathrm{e}{9}$ & $1.58\mathrm{e}{12}$ & $2.39\mathrm{e}{9}$ & $1.58\mathrm{e}{12}$ & $1.88\mathrm{e}{-20}$ \\
\cmidrule{1-9}
$6\mathrm{e}{19}$ & $0.006504$ & $3.84\mathrm{e}{6}$ & $3.64\mathrm{e}{9}$ & $3.64\mathrm{e}{9}$ & $2.60\mathrm{e}{12}$ & $2.75\mathrm{e}{9}$ & $2.60\mathrm{e}{12}$ & $7.65\mathrm{e}{-21}$ \\
\cmidrule{1-9}
$1\mathrm{e}{20}$ & $0.006421$ & $4.41\mathrm{e}{6}$ & $5.49\mathrm{e}{9}$ & $5.48\mathrm{e}{9}$ & $3.78\mathrm{e}{12}$ & $3.04\mathrm{e}{9}$ & $3.78\mathrm{e}{12}$ & $3.95\mathrm{e}{-21}$ \\
\cmidrule{1-9}
$3\mathrm{e}{20}$ & $0.006264$ & $5.83\mathrm{e}{6}$ & $1.34\mathrm{e}{10}$ & $1.34\mathrm{e}{10}$ & $8.57\mathrm{e}{12}$ & $3.72\mathrm{e}{9}$ & $8.57\mathrm{e}{12}$ & $9.51\mathrm{e}{-22}$ \\
\cmidrule{1-9}
$6\mathrm{e}{20}$ & $0.006179$ & $6.87\mathrm{e}{6}$ & $2.39\mathrm{e}{10}$ & $2.39\mathrm{e}{10}$ & $1.46\mathrm{e}{13}$ & $4.19\mathrm{e}{9}$ & $1.46\mathrm{e}{13}$ & $3.87\mathrm{e}{-22}$ \\
\cmidrule{1-9}
$1\mathrm{e}{21}$ & $0.006122$ & $7.70\mathrm{e}{6}$ & $3.66\mathrm{e}{10}$ & $3.66\mathrm{e}{10}$ & $2.16\mathrm{e}{13}$ & $4.55\mathrm{e}{9}$ & $2.16\mathrm{e}{13}$ & $2.00\mathrm{e}{-22}$ \\
\bottomrule
\end{tabular}
\end{table*}


\noindent From this fit, we can compute the details of optimal model size and optimal dataset size (number of tokens) needed for compute levels of interest. 
These details are shown in~\Cref{tab:000004_scaling_law_fits:eval_loss_min_snr_avg:compute_optimal_training_details}.
From this table, we can draw several interesting conclusions.
\begin{enumerate}
    \item The \textbf{optimal tokens-per-parameter ratio $r^\ast$ decreases with compute budget $C$}.
    This has a potential to make diffusion models a lucrative option at higher compute levels.
    \item The \textbf{optimal tokens-per-parameter ratio for auto-regressive models is usually around $20$}~\cite{DBLP:journals/corr/abs-2203-15556}. 
    Relative to this reference point, the fitted diffusion-optimal ratios in our explored compute regime remain substantially larger.
    However, it is unclear whether this optimal tokens to parameters ratio is a valid apples-to-apples comparison between diffusion-based and auto-regressive approaches due to differences in modalities, tokenization methods, and other architectural and optimization differences.
    {\textcolor{red}{[Eeshan] Maybe add the discussion of whether the tokens to parameters ratio is apples-to-apples can go here.}}.
    \item However, assuming it is possible to compare data-efficiency of auto-regressive models and diffusion models using the optimal tokens-to-parameter rations, 
    Scaling law studies usually demonstrate that scaling laws saturate after a point.
    However, if we assume that scaling laws will continue to hold with exactly the same form as shown above, we can \textbf{plot the optimal token-per-parameter ratio $r^\ast$ as a function of compute budget $C$ and observe where this graph cuts the value of $r^\ast = 20$}.
    This value will tell the compute $C^\dagger$ at which diffusion achieves computational parity with its auto-regressive counterpart and we can further infer the optimal model size $N^\dagger$ and optimal dataset size $D^\dagger$ at that compute level. 
    Note that we can get analytical expressions of $N^\ast$, $D^\ast$, and $r^\ast$ from our scaling law fit and use those to plot $r^\ast$ vs. $C$.
    \textbf{Extrapolating this curve to reach $r^\ast = 20$ requires compute of $9.6794\,\mathrm{e}29$, or approximately $1.0\mathrm{e}\,30$}.
    The plot for this extrapolation is shown in~\Cref{fig:000004_scaling_law_fits:eval_loss_min_snr_avg:r_star_vs_C}. 
    At this compute, \textbf{the optimal model size is $N^\dagger = 8.9812\mathrm{e}\,13$ and the optimal dataset size is $1.7962\mathrm{e}\,15$ tokens}.
    This would amount to training a model that is $5000\times$ the size of the largest model that we trained.
    \item Note that a peculiarity of the shape of the isoFLOPs is that \textbf{the isoFLOPs tend to get flatter as the compute budget increases}. 
    To quantify this observation, we consider for each compute budget $C$ the loss value of $L^\ast + \epsilon$ where $L^\ast$ represents the optimal loss for that compute budget. 
    The isoFLOP shape dictates that there will be a range of values of model sizes $N^\prime$ and a range of values of dataset sizes $D^\prime$ while keeping compute budget fixed such that the corresponding loss $L^\prime$ satisfies: $L^\prime\in \left[L^\ast, L^\ast + \epsilon\right]$. 
    We choose $\epsilon = 1\mathrm{e}-3$ for the sake of illustration.
    A characterization of the isoFLOPs getting flatter is that the aforesaid range of model sizes and dataset sizes gets bigger.
    This can be further quantified by computing the curvature of the isoFLOP at its optimum. 
    The results can be found in~\Cref{tab:000004_scaling_law_fits:eval_loss_min_snr_avg:scaling_law_fits_curvature}. 
    The results indicate that \textbf{as compute budget increases, isoFLOP curvature at the optimum point decreases}. 
    Consequently, \textbf{as compute budget increases, the range of model sizes and dataset sizes adhering to that compute budget such that they lead to a loss close enough to the optimum loss possible increases significantly}.
    This is a desirable quality in that at higher computes, to achieve a loss close enough to the optimum loss possible, a wide range of model sizes and dataset sizes is good enough to achieve a loss that is very close to the optimum loss.
\end{enumerate}


\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{plotting/000004_scaling_law_fits/PhonemeCoverageDivergence_1gram_JSD/cfg_2/isoflop_curves_vs_D.png}
    \hfill
    \includegraphics[width=0.49\textwidth]{plotting/000004_scaling_law_fits/PhonemeCoverageDivergence_1gram_JSD/cfg_4/isoflop_curves_vs_D.png}
    \caption{
        Scaling law fits with two-step fused scaling law for 1-gram pJSD.
    }
    \label{fig:000004_scaling_law_fits:PhonemeCoverageDivergence_1gram_JSD:two-step-fused-scaling-law}
\end{figure*}


\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{plotting/000004_scaling_law_fits/PhonemeCoverageDivergence_2gram_JSD/cfg_2/isoflop_curves_vs_D.png}
    \hfill
    \includegraphics[width=0.49\textwidth]{plotting/000004_scaling_law_fits/PhonemeCoverageDivergence_2gram_JSD/cfg_4/isoflop_curves_vs_D.png}
    \caption{
        Scaling law fits with two-step fused scaling law for 2-gram pJSD.
    }
    \label{fig:000004_scaling_law_fits:PhonemeCoverageDivergence_2gram_JSD:two-step-fused-scaling-law}
\end{figure*}


\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{plotting/000004_scaling_law_fits/PhonemeCoverageDivergence_3gram_JSD/cfg_2/isoflop_curves_vs_D.png}
    \hfill
    \includegraphics[width=0.49\textwidth]{plotting/000004_scaling_law_fits/PhonemeCoverageDivergence_3gram_JSD/cfg_4/isoflop_curves_vs_D.png}
    \caption{
        Scaling law fits with two-step fused scaling law for 3-gram pJSD.
    }
    \label{fig:000004_scaling_law_fits:PhonemeCoverageDivergence_3gram_JSD:two-step-fused-scaling-law}
\end{figure*}


\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{plotting/000004_scaling_law_fits/PhonemeCoverageDivergence_4gram_JSD/cfg_2/isoflop_curves_vs_D.png}
    \hfill
    \includegraphics[width=0.49\textwidth]{plotting/000004_scaling_law_fits/PhonemeCoverageDivergence_4gram_JSD/cfg_4/isoflop_curves_vs_D.png}
    \caption{
        Scaling law fits with two-step fused scaling law for 4-gram pJSD.
    }
    \label{fig:000004_scaling_law_fits:PhonemeCoverageDivergence_4gram_JSD:two-step-fused-scaling-law}
\end{figure*}


\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{plotting/000004_scaling_law_fits/PhonemeCoverageDivergence_5gram_JSD/cfg_2/isoflop_curves_vs_D.png}
    \hfill
    \includegraphics[width=0.49\textwidth]{plotting/000004_scaling_law_fits/PhonemeCoverageDivergence_5gram_JSD/cfg_4/isoflop_curves_vs_D.png}
    \caption{
        Scaling law fits with two-step fused scaling law for 5-gram pJSD.
    }
    \label{fig:000004_scaling_law_fits:PhonemeCoverageDivergence_5gram_JSD:two-step-fused-scaling-law}
\end{figure*}


\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{plotting/000004_scaling_law_fits/MetaAudioBoxAesthetics_CE/cfg_2/isoflop_curves_vs_D.png}
    \hfill
    \includegraphics[width=0.49\textwidth]{plotting/000004_scaling_law_fits/MetaAudioBoxAesthetics_CE/cfg_4/isoflop_curves_vs_D.png}
    \caption{
        Scaling law fits with two-step fused scaling law for content enjoyment (CE) component of MetaAudioBoxAesthetics.
    }
    \label{fig:000004_scaling_law_fits:MetaAudioBoxAesthetics_CE:two-step-fused-scaling-law}
\end{figure*}


\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{plotting/000004_scaling_law_fits/MetaAudioBoxAesthetics_CU/cfg_2/isoflop_curves_vs_D.png}
    \hfill
    \includegraphics[width=0.49\textwidth]{plotting/000004_scaling_law_fits/MetaAudioBoxAesthetics_CU/cfg_4/isoflop_curves_vs_D.png}
    \caption{
        Scaling law fits with two-step fused scaling law for content understanding (CU) component of MetaAudioBoxAesthetics.
    }
    \label{fig:000004_scaling_law_fits:MetaAudioBoxAesthetics_CU:two-step-fused-scaling-law}
\end{figure*}


\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{plotting/000004_scaling_law_fits/MetaAudioBoxAesthetics_PQ/cfg_2/isoflop_curves_vs_D.png}
    \hfill
    \includegraphics[width=0.49\textwidth]{plotting/000004_scaling_law_fits/MetaAudioBoxAesthetics_PQ/cfg_4/isoflop_curves_vs_D.png}
    \caption{
        Scaling law fits with two-step fused scaling law for production quality (PQ) component of MetaAudioBoxAesthetics.
    }
    \label{fig:000004_scaling_law_fits:MetaAudioBoxAesthetics_PQ:two-step-fused-scaling-law}
\end{figure*}


\subsubsection{Scaling Law for Phoneme Jensen-Shannon Divergence Metric (pJSD)}
\label{sec:temporary-devlog-fitting-scaling-laws:scaling-law-for-phoneme-jensen-shannon-divergence-metric-pJSD}
\noindent Fitting scaling laws for downstream metrics evaluating trained models is an interesting but tough challenge on which substantial progress has been made~\cite{DBLP:conf/iclr/Isik00PVK25,DBLP:journals/corr/abs-2512-08894}.
We begin by listing on two major approaches that have been tried in previous works.
\begin{enumerate}
    \item \textbf{Two-Step Fused Scaling Law}: This first approach advocates to plot the downstream metric against the validation loss of the model and infer a model function that can map validation loss to the metric value.
    If this function turns out to be well-defined and invertible, one can then apply the inverse of that function to the metric at hand, thereby transforming it into a variable that ought to have a scaling law fit whose expression would match the scaling law for the validation loss.
    The fitting of the function map and the fitting of the scaling law comprise the two steps required for fitting a scaling law this way, and hence the name of the approach. 
    However, to avoid unnecessary propagation of error, we rather fit both these functions jointly than fit separately.
    Thus, we call our first approach two-step fused scaling law, following prior two-step formulations used to relate scaling behavior of proxy training metrics to downstream outcomes~\cite{DBLP:journals/corr/abs-2107-03374,DBLP:journals/corr/abs-2412-04403}.
    \item \textbf{One-Step Scaling Law}: Recent work by Amitis et al. {\textcolor{red}{[Eeshan] Add citation}} on downstream scaling laws advocates transforming given downstream metric into its negative logarithm after having normalized the metric value using a random performance baseline~\cite{DBLP:journals/corr/abs-2512-08894}. 
    We also attempted this approach in our scaling laws fitting but we observed that the optimization was difficult to carry out. [Here, the actual issue was that either A or B coefficients in the scaling law fitting were hitting optimization boundary despite low MRE values. Amitis, what should we be doing here?]
\end{enumerate}
\noindent With these approaches we obtain scaling law fits with an acceptable MRE for the validation set~\cite{DBLP:journals/corr/abs-2512-08894}. 
However, revealing the exact scaling law for downstream metrics, especially when they have stochasticity in them, still remains an open challenge.


\subsubsection{Scaling Law for Admissible MetaAudioBoxAesthetics components}
\label{sec:temporary-devlog-fitting-scaling-laws:scaling-law-for-admissible-metaaudioboxaesthetics-components}
\noindent We follow the same two approaches for fitting scaling laws for the three components of MetaAudioBoxAesthetics which show desired isoFLOP behavior.
One of the major reasons to consider scaling law fitting on this metric is that for this metric, \textbf{we know baselines}; here, baselines refer to the metric values that were obtained by real audios. 
Thus, plotting scaling laws and extrapolating them has the potential to get a handle on how much more compute is needed to achieve metric values of real audios, thereby hinting at the possibility of realistic speech generation.


\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{plotting/000004_scaling_law_fits/MetaAudioBoxAesthetics_PQ/cfg_2/isoflop_curves_vs_D.png}
    \hfill
    \includegraphics[width=0.49\textwidth]{plotting/000004_scaling_law_fits/MetaAudioBoxAesthetics_PQ/cfg_4/isoflop_curves_vs_D.png}
    \caption{
        Scaling law fits with two-step fused scaling law for production quality (PQ) component of MetaAudioBoxAesthetics.
    }
    \label{fig:000004_scaling_law_fits:MetaAudioBoxAesthetics_PQ:two-step-fused-scaling-law}
\end{figure*}


\noindent Using the best fit that we found, we observe that \textbf{the optimal metric value for MetaAudioBoxAesthetics components that demonstrate scaling behavior can NOT reach the baseline metric values on real data no matter how much we scale up the compute}, thereby hinting at the possibility that we need systematic changes to speech-only language modeling and that our current setup may NOT be sufficient.
Even though this conclusion seems strong, we note that this claim must be tempered down in view of the following directions for future work.
\begin{enumerate}
    \item \textbf{Better scaling laws fitting:} Investigating \textbf{better functional form fit for downstream metrics of audio models} is going to be crucial.
    We wish to mention that \textbf{the aforesaid conclusions about attaining baseline metric values are strictly based on the best functional form we find and thus, it is possible that experimenting at a wider range of computes and fitting more accurate functional forms for scaling law may reveal different conclusions}.
    \item \textbf{Better inductive biases for SLMs:} On the other hand, if it turns out that speech-only models may NOT achieve baseline metrics on the real audio data no matter how much we scale up the compute, then it signifies that we may need better inductive biases, or even text-based conditioning inputs, to aid representation learning capabilities of SLMs.
\end{enumerate}


\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{plotting/000004_scaling_law_fits/MetaAudioBoxAesthetics_CU/cfg_2/Y_star_vs_C.png}
    \hfill
    \includegraphics[width=0.49\textwidth]{plotting/000004_scaling_law_fits/MetaAudioBoxAesthetics_CU/cfg_4/Y_star_vs_C.png}
    \caption{
        Plots of optimal MetaAudioBoxAesthetic metric component value $Y^\ast$ as a function of compute $C$.
        For brevity, we only plot the content understanding (CU) component but the trend is observed in other admissible components as well. 
        We observe that no matter how much we scale up the compute, we may NOT be able to attain the baseline metric value on real data.
    }
    \label{fig:000004_scaling_law_fits:MetaAudioBoxAesthetics_CU:Y_star_vs_C}
\end{figure*}


==> body/98_temporary_devlog_isoFLOPs_analysis.tex <==
\clearpage
\subsection{[Temporary][Devlog] isoFLOP Analysis}
\label{sec:temporary-devlog-isoFLOP-analysis}
% Validation loss.
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/eval_loss_min_snr_avg/cfg_2_filter_default.png}
    \hfill
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/eval_loss_min_snr_avg/cfg_4_filter_default.png}
    \caption{
        Validation loss isoFLOPs.
    }
    \label{fig:000003_isoFLOPs:eval_loss_min_snr_avg}
\end{figure*}


% MetaAudioBoxAesthetics::CE
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/MetaAudioBoxAesthetics_CE/cfg_2_filter_default.png}
    \hfill
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/MetaAudioBoxAesthetics_CE/cfg_4_filter_default.png}
    \caption{
        MetaAudioBoxAesthetics: Content Enjoyment isoFLOPs.
    }
    \label{fig:000003_isoFLOPs:MetaAudioBoxAesthetics::CE}
\end{figure*}


% MetaAudioBoxAesthetics::CU
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/MetaAudioBoxAesthetics_CU/cfg_2_filter_default.png}
    \hfill
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/MetaAudioBoxAesthetics_CU/cfg_4_filter_default.png}
    \caption{
        MetaAudioBoxAesthetics: Content Understanding isoFLOPs.
    }
    \label{fig:000003_isoFLOPs:MetaAudioBoxAesthetics::CU}
\end{figure*}

% MetaAudioBoxAesthetics::PC
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/MetaAudioBoxAesthetics_PC/cfg_2_filter_default.png}
    \hfill
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/MetaAudioBoxAesthetics_PC/cfg_4_filter_default.png}
    \caption{
        MetaAudioBoxAesthetics: Production Complexity isoFLOPs.
    }
    \label{fig:000003_isoFLOPs:MetaAudioBoxAesthetics::PC}
\end{figure*}

% Does PQ make sense for us? The plots don't show much
% MetaAudioBoxAesthetics::PQ
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/MetaAudioBoxAesthetics_PQ/cfg_2_filter_default.png}
    \hfill
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/MetaAudioBoxAesthetics_PQ/cfg_4_filter_default.png}
    \caption{
        MetaAudioBoxAesthetics: Production Quality isoFLOPs.
    }
    \label{fig:000003_isoFLOPs:MetaAudioBoxAesthetics::PQ}
\end{figure*}


% PhonemeCoverageDivergence::1gram::JSD
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/PhonemeCoverageDivergence_1gram_JSD/cfg_2_filter_default.png}
    \hfill
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/PhonemeCoverageDivergence_1gram_JSD/cfg_4_filter_default.png}
    \caption{
        PhonemeCoverageDivergence JSD on 1-grams isoFLOPs.
    }
    \label{fig:000003_isoFLOPs:PhonemeCoverageDivergence::1gram::JSD}
\end{figure*}


% PhonemeCoverageDivergence::2gram::JSD
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/PhonemeCoverageDivergence_2gram_JSD/cfg_2_filter_default.png}
    \hfill
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/PhonemeCoverageDivergence_2gram_JSD/cfg_4_filter_default.png}
    \caption{
        PhonemeCoverageDivergence JSD on 2-grams isoFLOPs.
    }
    \label{fig:000003_isoFLOPs:PhonemeCoverageDivergence::2gram::JSD}
\end{figure*}


% PhonemeCoverageDivergence::3gram::JSD
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/PhonemeCoverageDivergence_3gram_JSD/cfg_2_filter_default.png}
    \hfill
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/PhonemeCoverageDivergence_3gram_JSD/cfg_4_filter_default.png}
    \caption{
        PhonemeCoverageDivergence JSD on 3-grams isoFLOPs.
    }
    \label{fig:000003_isoFLOPs:PhonemeCoverageDivergence::3gram::JSD}
\end{figure*}


% PhonemeCoverageDivergence::4gram::JSD
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/PhonemeCoverageDivergence_4gram_JSD/cfg_2_filter_default.png}
    \hfill
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/PhonemeCoverageDivergence_4gram_JSD/cfg_4_filter_default.png}
    \caption{
        PhonemeCoverageDivergence JSD on 4-grams isoFLOPs.
    }
    \label{fig:000003_isoFLOPs:PhonemeCoverageDivergence::4gram::JSD}
\end{figure*}


% PhonemeCoverageDivergence::5gram::JSD
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/PhonemeCoverageDivergence_5gram_JSD/cfg_2_filter_default.png}
    \hfill
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/PhonemeCoverageDivergence_5gram_JSD/cfg_4_filter_default.png}
    \caption{
        PhonemeCoverageDivergence JSD on 5-grams isoFLOPs.
    }
    \label{fig:000003_isoFLOPs:PhonemeCoverageDivergence::5gram::JSD}
\end{figure*}


% NB(jramapuram): These results dont show much. Removing
% DNSMOS::P808_MOS
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/DNSMOS_P808_MOS/cfg_2_filter_default.png}
    \hfill
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/DNSMOS_P808_MOS/cfg_4_filter_default.png}
    \caption{
        DNSMOS P808-MOS isoFLOPs.
    }
    \label{fig:000003_isoFLOPs:DNSMOS::P808_MOS}
\end{figure*}

% NB(jramapuram): These results dont show much. Removing
% NISQA::MOS
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/NISQA_MOS/cfg_2_filter_default.png}
    \hfill
    \includegraphics[width=0.49\textwidth]{plotting/000003_isoFLOPs/NISQA_MOS/cfg_4_filter_default.png}
    \caption{
        NISQA MOS isoFLOPs.
    }
    \label{fig:000003_isoFLOPs:NISQA::MOS}
\end{figure*}

% % [Eeshan]: Added the gist of devlog into the main body. Commenting.
To explore and validate scaling laws, we train models varying the number of parameters $N \in \{A, B, C, D\}$ and dataset sizes $D \in \{E, F, G, H\}$, maintaining constant computational resources defined by $C = 6ND$. In~\autoref{fig:000003_isoFLOPs:eval_loss_min_snr_avg}, we present isoFLOP experiments~\cite{kaplan2020scaling,DBLP:journals/corr/abs-2203-15556} for the Min-SNR training objective~\eqref{eq:minsnr_loss}. Unlike prior research~\cite{DBLP:journals/corr/abs-2410-08184} conducted in the latent space of a Variational Autoencoder, our methodology operates directly on raw speech data represented by Mel filterbanks. We observe a clear trend the elucidates the existence of a compute optimal raw speech diffusion transformer and fit a scaling law: $L(N, D) = E + (A/D^\alpha + B/N^\beta)^\gamma $ which results in $E=..., A=...$.

A key contribution of this work is the validation of scaling laws in downstream performance metrics. \autoref{fig:000003_isoFLOPs:PhonemeCoverageDivergence::3gram::JSD} demonstrates scaling behavior in the phoneme Jensen-Shannon Divergence (JSD) metric (~\autoref{sec:phoneme-jsd}). Additionally as in [CITE JAKUB, AMITIS PAPER], we identify scaling laws for Meta Audiobox content enjoyment (\autoref{fig:000003_isoFLOPs:MetaAudioBoxAesthetics::CU}) and content usefulness metrics (\autoref{fig:000003_isoFLOPs:MetaAudioBoxAesthetics::CE}).

\textbf{Note(Jramapuram): this entire section is far too verbose and should not be included. I have added a truncated section above that conveys this in two paragraphs. }

\noindent Below are some of the points that will be worth highlighting based on our syncs. 
\begin{enumerate}
    \item \textbf{isoFLOP curves} are generated by plotting the validation loss or other downstream metrics versus dataset size $D$ or model size (number of non-embedding trainable parameters) $N$. 
    To plot an isoFLOP curve for compute $C$, we consider different pairs $(N, D)$ that result in this compute budget of $C$ using compute approximation $C \approx 6\cdot N\cdot D$~\cite{DBLP:journals/corr/abs-2203-15556}. 
    For each such setting of $(N, D)$, we train a model, compute its validation loss and evaluate downstream metrics on it. 
    Plotting these values against either $N$ or $D$ give the isoFLOP curve for that compute value $C$.
    We plot isoFLOP curves for computes ranging from $1.0\textrm{e}+18$ to $6.0\textrm{e}+20$. 
    \item For revealing scaling laws for the validation loss and downstream metrics, we first need to see which of these demonstrate an \textbf{expected isoFLOP behavior}, which consists of two aspects: \emph{1.} the shape of isoFLOP curves, \emph{2.} the effect of compute budget $C$ on isoFLOP curves.
    At any compute level $C$, there are two extremes of $(N, D)$ settings for that compute: \emph{i.} low $N$ and high $D$ settings, which correspond to underparametrized models that are overtrained, and \emph{ii.} high $N$ and low $D$ settings, which correspond to overparametrized models that are undertrained.
    We expect that in the former case, the underparametrized models would not posses the capacity to learn meaningful data representations no matter the amount of compute. 
    Similarly, in the latter case, the overparametrized models without enough data can not learn meaningful data representations as well. 
    Thus, we expect that at both the extremes of $(N, D)$ settings of any fixed compute level $C$, the validation loss or downstream metric values should be poorer.
    Consequently, we expect to see a golden middle at which we can have optimally sized models that are trained on optimally sized dataset so that the metrics of interest are optimal, which we refer to as expected isoFLOP behavior. 
    Concretely, \textbf{for validation loss and downstream metrics that are ``the lower the better'', we expect the isoFLOPs to be $\cup-$shaped curves} and \textbf{for other downstream metrics that are ``the higher the better'', we expect the isoFLOPs to be $\cap-$shaped curves}. 
    Further, note that if we increase our compute budget $C$, we can expect same sized models to be trained on more data so as to satisfy the new compute budget.
    Thus, \textbf{we expect isoFLOPs of higher compute budgets to lead to a more optimal metric compared to the isoFLOPs of smaller compute budgets}.
    As we discuss later, observing this expected isoFLOP behavior for a metric allows us to expect a reliable scaling law fit for it. 
    \item From Figure~\ref{fig:000003_isoFLOPs:eval_loss_min_snr_avg}, we see that the validation loss indeed demonstrates expected isoFLOP behavior and thus, we expect a scaling law fit for the validation loss of audio diffusion models.
    Our observations of expected isoFLOP behavior for the validation loss complement the findings of~\cite{DBLP:journals/corr/abs-2410-08184}, where analogous investigations are carried out for diffusion transformers and for discrete diffusion models respectively. 
    \item From Figures~\ref{fig:000003_isoFLOPs:PhonemeCoverageDivergence::1gram::JSD},~\ref{fig:000003_isoFLOPs:PhonemeCoverageDivergence::2gram::JSD},~\ref{fig:000003_isoFLOPs:PhonemeCoverageDivergence::3gram::JSD},~\ref{fig:000003_isoFLOPs:PhonemeCoverageDivergence::4gram::JSD}, and~\ref{fig:000003_isoFLOPs:PhonemeCoverageDivergence::5gram::JSD}, we see that the Phoneme Jensen-Shannon Divergence (pJSD) metric described in Section~\ref{sec:phoneme-jsd}, which is of the type ``the-lower-the-better'' also demonstrates the desired isoFLOP behavior. 
    \item Interestingly, most of the speech perception quality metrics do NOT demonstrate the expected isoFLOP behavior, except for three of the four Meta AudioBox Aesthetics components-- content enjoyment (CE), content understanding (CU), and production quality (PQ); the remaining component of production complexity (PC) does NOT demonstrate the expected isoFLOP behavior. 
    \item We hypothesize that \textbf{the lack of observing desired scaling behavior might be caused because the underlying metric might already be saturated}; that is, with the compute levels that we experimented with, all models that we trained and evaluated have already learned the respective features to a great extent so much so that the metric values are already very close to their optimal values. 
    To test this hypothesis, we compute these speech perceptual quality metrics for the ground truth data and plot those as the baseline value for the models to achieve. 
    From the isoFLOP plots with baselines for DNSMOS (P808-MOS) from Figure~\ref{fig:000003_isoFLOPs:DNSMOS::P808_MOS}, NISQA (MOS) from Figure~\ref{fig:000003_isoFLOPs:NISQA::MOS}, and the production complexity component (PC) from Figure~\ref{fig:000003_isoFLOPs:MetaAudioBoxAesthetics::PC}, we can see that this seems to be indeed the case; \textbf{all the isoFLOP plots support the observation that metrics that are already saturated near their baselines do NOT show the desired scaling behavior}.
    Here, saturated near the baseline would mean that the mean of the metrics is within one standard deviation of the baseline value.
    Thus, the expected isoFLOP behavior is not unexpected. 
    \item If we observe the expected scaling behavior in the loss and/or in the downstream metrics, we can have a higher confidence that we can fit a scaling law for these entities. 
    This is so because we know that as compute scales up, we can expect a better metric value, which depends on the dataset size $D$ and the model size $N$. 
\end{enumerate}

==> templates/apple/math_commands.tex <==
%%%%% Renark: do not use
%%%%% Inherited from Apple template

%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

